Signatures of links and finite type invariants of cyclic branched covers

Recently, Mullins calculated the Casson-Walker invariant of the 2-fold cyclic branched cover of an oriented link in S^3 in terms of its Jones polynomial and its signature, under the assumption that the 2-fold branched cover is a rational homology 3-sphere. Using elementary principles, we provide a similar calculation for the general case. In addition, we calculate the LMO invariant of the p-fold branched cover of twisted knots in S^3 in terms of the Kontsevich integral of the knot.

==> draws/Aray.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(2544,2133)(0,-10)
\thicklines
\path(12,12)(1512,612)
\path(1411.725,539.579)(1512.000,612.000)(1389.441,595.287)
\path(12,12)(1812,1212)
\path(1728.795,1120.474)(1812.000,1212.000)(1695.513,1170.397)
\path(12,12)(1512,1512)
\path(1448.360,1405.934)(1512.000,1512.000)(1405.934,1448.360)
\path(12,12)(612,1812)
\path(602.513,1688.671)(612.000,1812.000)(545.592,1707.645)
\path(12,12)(1812,312)
\path(1698.565,262.680)(1812.000,312.000)(1688.701,321.864)
\put(462,1962){\makebox(0,0)[lb]{$A_r$}}
\put(1737,612){\makebox(0,0)[lb]{$A_0= 1 = \b_2$}}
\put(2037,1137){\makebox(0,0)[lb]{$A_1$}}
\put(1662,1587){\makebox(0,0)[lb]{$A_2$}}
\put(612,1287){\makebox(0,0)[lb]{$\cdots$}}
\put(1962,162){\makebox(0,0)[lb]{$A_{-1}=w_0 = \b_1$}}
\end{picture}

